Local Embeddings for Relational Data Integration

Deep learning based techniques have been recently used with promising results for data integration problems. Some methods directly use pre-trained embeddings that were trained on a large corpus such as Wikipedia. However, they may not always be an appropriate choice for enterprise datasets with custom vocabulary. Other methods adapt techniques from natural language processing to obtain embeddings for the enterprise's relational data. However, this approach blindly treats a tuple as a sentence, thus losing a large amount of contextual information present in the tuple. We propose algorithms for obtaining local embeddings that are effective for data integration tasks on relational databases. We make four major contributions. First, we describe a compact graph-based representation that allows the specification of a rich set of relationships inherent in the relational world. Second, we propose how to derive sentences from such a graph that effectively "describe" the similarity across elements (tokens, attributes, rows) in the two datasets. The embeddings are learned based on such sentences. Third, we propose effective optimization to improve the quality of the learned embeddings and the performance of integration tasks. Finally, we propose a diverse collection of criteria to evaluate relational embeddings and perform an extensive set of experiments validating them against multiple baseline methods. Our experiments show that our framework, EmbDI, produces meaningful results for data integration tasks such as schema matching and entity resolution both in supervised and unsupervised settings.

==> response.tex <==
\renewcommand{\ni}{\noindent}
\newcommand{\stab}{\vspace{1.2ex}\noindent}
\newcommand{\etitle}[1]{\vspace{0.8ex}\noindent{\underline{\em #1}}}
\newcommand{\red}[1]{\textcolor{red}{#1}}

%\begin{center}
%\section*{Responses to Reviewers for PaperID: 529}
%\subsection*{Creating Embeddings of Heterogeneous Relational Datasets for Data Integration Tasks}
%\end{center}
\twocolumn [\begin{center}\huge{\textbf{SIGMOD 2020 Paper 529: Author Response to Reviews of \\{\em Creating Embeddings of Heterogeneous Relational Datasets for Data Integration Tasks}}}\end{center}\vspace{8ex}]

\ni {\bf{\em Dear SIGMOD Reviewers:}}

\stab
We thank the reviewers for their insightful comments, based on which we have made significant changes to improve the paper. The new material in the paper is highlighted in \rev{blue}. We start with a description of our major changes.

%METAREVIEW
%Please address R2:D1,D3; R4:D1,D2,D3; and R5:D1,D2.
%The reviewers were mostly satisfied with the revisions proposed in the feedback with one exception. For R4:D1, reviewers felt that the claim that "methods based on embeddings outperform previous techniques in data integration tasks" is not entirely accurate, based on results reported in "Deep Learning for Entity Matching" (SIGMOD18, Table 3). The Fodors-Zagats restaurant dataset is known to be easy (with F-score=1 for feature-based methods). We encourage the authors to use more difficult benchmark data from the literature (e.g., more difficult datasets from SIGMOD18).

\stab
{\bf C1.}\label{section:C1}
We extended the experimental campaign with six datasets form the literature~\cite{deepmatcher,DasCDNKDARP17}.
Experimental results confirm the efficacy of our local embeddings for entity resolution and schema matching.


%The quality results are aligned with those for smaller datasets, thus confirming that our approach scales effectively with 1M tuples. As MSD has only one table, we do not report SM and ER results, but our embeddings could be used for these tasks.
%\red{Paolo: quite poor justification, but the real details are that SM is not possible (only one dataset) and ER is messy as MSD is the integration of 7 datasets! there are 1.4M matches, we will never find them with our current algorithm. Moreover, it's very messy, in fact they used it in a paper with crowd...maybe we can give these details instead of my fluffy answer}



\stab
{\bf C2.} The tokenization strategy is a key step in the graph construction process.
We now better clarify how we tokenize cell values and report experimental results with three different strategies. 
%The new datasets are more noisy than the ones that we originally consider in our experiments. For example, product records often report name and description of items across different attributes without a consistent division of the keywords. Also, such datasets contain longer text descriptions, making node merging harder than when dealing with one or two words in a cell value. This has motivated us to model at a finer granularity the cell values that are not overlapping or merged across two datasets in data integration scenarios. This means that if a cell value for tuple $t$ and attribute $a$ for the first dataset reports ``iPad 4th" and the token is not merged with any token in the second dataset, then we model its single words directly in our graph with two nodes (``iPad'', ``4th") associated to both $t$ and $a$. This small change to the graph construction does not require any modification to the other steps of our workflow but delivers great results in terms of quality improvement. 
%This distinction is now more clear across the paper, with a new version of Figure 1 and the corresponding graph in Figure 2. These clarifications also addresses comment D1 from Reviewer 5.



\stab
{\bf C3.} We have formalized the discussion of our technical material. Specifically, we have added five additional pseudocodes to describe the various components and algorithms for unsupervised entity and schema matching using our embeddings.

\stab
{\bf C4.} We addressed all the minor issues and introduced several clarifications in terms of presentation. 

\vspace{4ex}
\section*{Responses to the Comments of Reviewer 2.}


\vspace{0.8ex}
\etitle{R2(D1).}
{\em The descriptions on Section 4 and 5 (i.e., the algorithm to learn word embeddings as well as the techniques used to improve learning) are too sketchy. The content in those two sections are well structured and the authors use a lot of space to motivate the design choices, both of which are very helpful for people to understand better. However, when going into the technical details, it’s getting vague, i.e., key algorithmic procedures on the proposed method are missing from the paper. Without these it will be very hard for people to implement the method and reproduce the results. I suggest the authors to provide more algorithmic details, e.g., how the graph is traversed, how the random walks are performed, etc.}

\stab
{\bf [A]}
We have made a number of changes to address the comment.
We have added five new pseudocodes to describe the various components in detail.
These include graph generation (Algorithm~1), random walk (Algorithm~2) and embedding alignment (Algorithm~4).
Furthermore, we have added details about how the data integration tasks could be performed using the local embeddings (Algorithms~5 and~6).
%describe how Schema matching and Entity matching could be done using our embeddings.
In the experiment section, we now describe better how the algorithmic details in Sections 4 and 5 were instantiated.
Finally, an anonymized link to the code can be found at \url{http://pc.cd/SRj}.
If our paper is accepted, we plan to release the code as a Python package to be used by the community.


\vspace{0.8ex}
\etitle{R2(D2).}
{\em the authors conduct extensive evaluation to support their claims. However, maybe it is too crowded to fit many experiments in the paper, the description of each part is a bit hasty and not easy to follow. I would recommend the authors the reorganize the experiment section to give a clear explanation on each task. If it goes beyond the page limit, some of them may be removed and put in a technical report.}


\stab
{\bf [A]}
We have performed an extensive rewrite of the experiment section.
We now spell out more clearly the 3 fundamental questions that the section answers:
\begin{enumerate}
    \item did our proposed embeddings learn the major relationships inherent in structured data?
    \item how well do our embeddings behave in multiple data integration tasks, under supervised and unsupervised conditions?
    \item what are the contributions of our design choices?
\end{enumerate}
We believe that the new version reinforces the central message that our proposed approach for learning local embeddings can be used to improve deep learning-based approaches for data integration.
We have also added further details about the setting and the outcome of every experiment
so that they are more easily followed.

\vspace{0.8ex}
\etitle{R2(D3).}
{\em Some important experiments are missing from the paper. For example, the datasets shown in table 1 are pretty small. I wonder how the algorithm will scale (in terms of runtime and memory usage) given some large datasets (e.g., with 1M tuples in a single table). Also, there are many publicly available datasets for the evaluated tasks. The authors should try more to make the claims convincing.}

\stab
{\bf [A]}
In our original submission, we conducted experiments on three datasets -- IMDB-Movielens (IM), DBLP-ACM (DA), DBLP-Scholar (DS). 
These were exemplars for the practical real-world issues that necessitated our design choices.
In our revised version, we have conducted experiments over six new datasets, namely 
Amazon-Google (AG), Walmart-Amazon (WA), Itunes-Amazon (IA), Fodors-Zagats (FZ),   BeerAdvo-RateBeer (BB), and Million Songs Dataset (MSD), which has 1M tuples in one table.
We believe that the additional datasets show that our proposed approaches 
can perform well on diverse datasets and can readily scale.

In terms of memory consumption, we have been able to run all tests, including the ones for the biggest dataset of 1M tuples, even in a laptop with 16GB of main memory. We report faster results in terms of execution times compared to the original submission because of improvements to our codebase. Finally, we would like to note that the key steps in our algorithms are either
embarrassingly parallel (random walks) or extremely scalable (embedding alignment).


%\red{Sara: Should we chose from structured datasets or textual/dirty ones?????}
%\red{Paolo: we picked only from the structured ones - we may mention somewhere that we plan to study further how to deal with noise and long texts}

\section*{Responses to the Comments of Reviewer 4.}
\vspace{0.8ex}
\etitle{R4(D1a).}
{\em First, current results are reported on 3 data sets (2 public ones known to be easy from the bibliographic domain, 1 newly created by the authors). With decades of literature on data integration, there are tens of well-known data sets for entity resolution and schema matching widely used by prior work to report quality numbers. It is not entirely clear why a new data set needs to be created for the tasks, and among the known benchmark data sets only 2 bibliographic data sets are used in the experiments. If the authors can report quality numbers on benchmark data sets from the literature, it would help to better establish the benefit of the proposed method.}



\stab
{\bf [A]}
We have conducted  experiments on six additional datasets -- 
Amazon-Google (AG), Walmart-Amazon (WA), Itunes-Amazon (IA), Fodors-Zagats (FZ),   BeerAdvo-RateBeer (BB), Million Songs Dataset (MSD).
Based on your and Reviewer 2's suggestions, these were chosen from the list of
structured datasets from Table~2 of DeepMatcher paper~\cite{deepmatcher}.
As mentioned in the DeepMatcher paper~\cite{deepmatcher}, 
four of the datasets from Table~2 came from a retailer and were not publicly available.
Hence, we performed experiments on the remaining datasets.
The experimental results show that our proposed embeddings provide good results on these new datasets and outperform pre-trained embeddings in all tasks. 

%\red{Should we chose from structured datasets or textual/dirty ones?????}


\vspace{0.8ex}
\etitle{R4(D1b).}
{\em Additionally, all comparisons seem to be performed against different variants of local embedding methods, which however are not known to excel in data integration tasks. It would be hard to judge the relative merit of proposed method without using methods from the data integration literature as reference points. Comparison with standard pre-trained embedding would also be useful (since all three data sets are already from the public domain).}

\stab
{\bf [A]}
Indeed.
Embedding based approaches for data integration are not a panacea and may not always be the best choice.
The DeepMatcher paper~\cite{deepmatcher} shows (in Table~3) that for
structured datasets non-deep learning based approaches often outperform or provide competitive results.
%Embedding based approaches often excel for textual and dirty datasets.
Our contention is not that embedding methods always outperform prior approaches.
We believe that a bouquet of deep learning, machine learning and other approaches
is often needed for real-world data integration tasks.
In this context, we argue that naively using a pre-trained embeddings is sub-optimal.
The pre-trained are often trained using a large textual corpus for other downstream NLP tasks.
We believe that a local embedding approach would be able to learn the major relationships inherent in a structured dataset, thus providing better results.

Our experimental setup seeks to validate this hypothesis.
All of the prior work such as DeepER~\cite{deeper}, DeepMatcher~\cite{deepmatcher}
and Seeping Semantics~\cite{seepingSemantics} directly use pre-trained embeddings.
In Tables~3 and~4, we show that the variants of DeepER and Seeping Semantics
that use our local embeddings outperform those that use pre-trained embeddings.
In Table~2, we show that our proposal for learning local embeddings is superior
to existing graph embedding approaches in terms of embeddings quality. We now discuss the poor performance of pre-trained embeddings for this task.



\vspace{0.8ex}
\etitle{R4(D1c).}
{\em More specifically, the two bibliographic datasets (RefS and RefL) are also known to be easy with substantial overlapping values. Schema matching on these two data sets probably only require treating each column as a bag of words, and standard n-gram model can already get columns matched correctly. Similarly, for entity resolution, vanilla similarity join (with perhaps tf-idf weighting) should already work reasonably well on the two data sets. It is not entirely clear if sophisticated embedding is needed for the performance numbers reported.}

\stab
{\bf [A]}
We apologize for the confusion.
As before, our contention is not that embedding based approaches are always needed for data integration.
Indeed, for some bibliographic datasets, simple approaches for
schema matching and entity matching suffice.
With Tables~3 and~4, our objective is to show that prior embedding-based work for schema and entity matching provides better results when using our local embeddings compared to pre-trained embeddings.
Our new experiments on additional datasets from DeepMatcher show that this observation holds true for other difficult datasets.

\vspace{0.8ex}
\etitle{R4(D1d).}
{\em There are a few additional concerns on the design of token match experiment (what columns in Movie is used, how are ground-truth determined and prediction evaluated, whether the exercise can be carried out on RefS and RefL, etc.), and similarly, the embedding-quality experiment.}

\stab
{\bf [A]}
We agree that the original description was not clear enough and we have now explained better the experiment settings. 
Regarding the token matching experiment, we picked attributes for which we had ground truth, i.e., the list of synonyms was available. This requirement led us to columns such as countries and languages, as the list of alternative name encodings is available (e.g., ``USA'' vs ``United States of America'').
For the embedding quality experiment, we now better clarify how the tests have been generated.
%distinguish the three cases. For columns, we consider every attribute of the dataset and pick ``noise'' from a second attribute at random. For rows, we pick a random sample of rows. For concept, we manually pick pairs of columns that are in a semantic relationship, such as director and movie title. 

\vspace{0.8ex}
\etitle{R4(D2).}
{\em The authors mention enterprise settings repeatedly in the intro to motivate local training. The running example in Figure 1 feels a bit toyish for that purpose, however. Enterprise tables may have entirely different vocabularies not seen in public domains, where the effectiveness of local training on one table can be uncertain. The current experiments are all on tables from the public domain, where pre-trained embedding (e.g., Glove) may already be reasonable, and the benefit of local training is not entirely clear.}

\stab
{\bf [A]}
In our experiments, we used public domain datasets so that
we could fairly compare against pre-trained embeddings.
Our experimental results from Tables~3 and~4 show that it is beneficial to use
local embeddings if the downstream task is data integration.
This is not surprising as pre-trained embeddings were designed for NLP tasks.
On the other hand, local embeddings, such as those obtained with EDI, are tailored for data integration and would therefore provide better results in those tasks.
Similarly, as Table~2 shows, they can learn the major relationships in the structured data.
%\red{Sara: should we add an entry in Table~2 comparing one pretrained embedding?} \red{Paolo: we can do it by using average of the words for a cell value. However we anticipate that the results are going to be poor}
We anticipate that our approach can provide even better results for enterprise data
that contain words that might not be known to pre-trained embeddings such as fastText and GloVe.
Local embeddings learned on the data capture the enterprise specific semantics and
would show bigger improvements.


\etitle{R4(D3a).}
{\em The algorithm part for data integration is described only in Section 6. The algorithms described here are quite ad-hoc at places. For example, schema matching follows a random match procedure. It is not clear why such randomness is needed, and no analysis is given in terms of the guarantees it may have.}

\stab
{\bf [A]}
We have added five new pseudocodes in Sections 4-6 to describe the various components and algorithms in detail.
These include graph generation (Algorithm~1), random walk (Algorithm~2) and embedding alignment (Algorithm~4).
Furthermore, we have added details about how the data integration tasks could be performed using the local embeddings.
Specifically, Algorithms~5 and~6 describe how Schema matching and Entity matching could be done using our embeddings.

We would like to reiterate that our key contribution is a novel framework for generating local embeddings
that are optimized for data integration.
Prior work such as DeepER~\cite{deeper}, DeepMatcher~\cite{deepmatcher}, Seeping Semantics~\cite{seepingSemantics} and others improve their performance
by using our embeddings as against pre-trained embeddings.
This is shown in Tables 3 and 4 of our paper.
%Note that supervision in the form of training data is often widely used in data integration tasks.
%This can lead to better results by identifying irrelevant attributes
%and filtering them out in the decision step.
%In Tables~3 and~4, we discussed some simple unsupervised algorithms for schema and entity matching.
Our contention is not that our unsupervised algorithms always outperform  state-of-the-art methods.
Instead, our objective is to show that our training procedures learned enough data integration semantics
that the embeddings imbibe the notion of similar attributes (useful for schema matching) and
similar tuples (useful for entity matching).



\vspace{0.8ex}
\etitle{R4(D3b).}
{\em Similarly for entity resolution, it is only described that each row in one table is matched with top-``n'' rows from both tables, where top rows from the other table is regarded as matches. This parameter n would have a substantial impact on match accuracy, which however is not discussed. There are also entity resolution scenarios, where the two tables may have attributes with long textual fields, or many other attributes irrelevant to the matching decisions. It is not clear how the proposed method would be able to differentiate.}

\stab
{\bf [A]}
Our goal in Table~4 is to show that our embeddings have learned semantics
such as similar tuples and attributes.
The top-n is a simple test used by the NLP community to show that
pre-trained embeddings have learned semantic relationships between words.
This is usually done by showing that synonyms of a word appear among its top-n neighbors.
We conducted an equivalent test and showed that the
duplicate tuple was routinely among the top-n neighbors of a given tuple.
We have conducted a new experiment that evaluated the impact of $n$.
As shown in the new Table~5, our proposed approaches can give good results even for $n=1$.
%
%\red{We have added further details about how the parameter `n' affects the matching.}
%\textcolor{blue}{Sara: If n is something like 10, we can say this is obtained from NLP and not do any new experiments}
%\riccardo{Where should we explain the new testing method for ER? (the symmetry check)}
We would like to note that handling textual attributes is one of the scenarios where
embedding-based approaches outperform traditional approaches that are not based on embeddings.
%\riccardo{What do we mean by traditional? }
This phenomenon has been observed in other works, e.g., Table~3 of~\cite{deepmatcher}.

\section*{Responses to the Comments of Reviewer 5.}

\vspace{0.8ex}
\etitle{R5(D1).}
{\em In the case of multi-word cells, it is not clear if the entire sentence / word sequence treated as a single token, or if it is tokenized and token sequence is part of the generated random walk sentences. It'll be good to show examples of this case.}

%\stab
%{\bf [A]}
%In our current implementation, when a cell contains multiple words, such as ``Tom Hanks'',
%the preprocessing step replaces spaces with ``\_'' to model
%the cell value as a single word, e.g., ``Tom\_Hanks''.
%Given the sentence, most word (not character) embedding methods produce a vector per word,
%as they do not produce vectors for n-grams.
%While vectors for n-grams can be derived (e.g., by averaging the word vectors), they can be of low quality.
%Consider a movie title ``Saving Private Ryan''.
%Its embedding is the combination of 3 generic word embeddings that do not model the movie domain.
%We therefore choose a more accurate modeling, one vector for Tom\_Hanks and one for Tom\_Cruise.

%We have conducted additional experiments that show
%how the embeddings quality varies based on tokenization.
%Specifically, we consider two extremes.
%One where the entire word sequence is treated as a single token
%and the other where we tokenize the word sequence and then aggregate them.
%The results can be shown in Table~blah.
%Identifying an appropriate tokenization strategy is a challenging problem
%and is a key focus of our future investigation.

\stab
{\bf [A]} 
Indeed. There are a number of ways in which multi-word cells could be tokenized.
One simple option is to treat the entire word sequence as a single token.
The other option is to tokenize the word sequence, compute the word embeddings for each of the tokens, 
and then aggregate these token embeddings to get the embedding for the multi-word cell. 
There are two key problems: how to tokenize a multi-world cell and 
how to aggregate the token embeddings to get the cell embeddings.
There are no simple answers to this problem. 
%and is a key focus of our future investigation.

%Given a sentence, most word (not character) embedding methods produce a vector per word, as they do not produce vectors for n-grams.
%While vectors for n-grams can be derived (e.g., by averaging the word vectors), they can be of low quality, as we shown experimentally in \red{Table XYZ for method ABC}. 
Consider a movie title ``Saving Private Ryan''. Its embedding is the combination of 3 generic word embeddings that do not model precisely the movie domain. An accurate modeling is to have one vector for ``Saving Private Ryan'', obtained by concatenating the 3 words in one a single one, e.g., ``Saving\_Private\_Ryan''. This is the perfect solution for structured datasets where the domains are controlled and uniform to some extent.
On the other hand, a finer granularity is mandatory for long, heterogeneous texts. Consider again the same movie, but in a different dataset where is stored with title ``Saving Private Ryan (1998, USA)''.  A traditional solution is to use distance function, as we also support with our merge function. However, merging becomes more challenging with longer sequences of words, as it happens with some of the new datasets that we considered in the revision. Moreover, the same entities can be split in attributes or grouped in one attribute across different datasets. As an example, both beer datasets contain attributes ``beer name" and ``brewing company". However, in one dataset very often the name of the brewing company appears in the beer name "brewing\_company\_A beer\_name\_1", while in the other dataset only beer\_name\_1 appears in the name column. As we do not assume any user-defined preprocessing of the attribute values, modeling the words (of a cell value) individually is beneficial in these cases. This is especially true in our graph based approach where we target ER and SM as applications. As our goal is to model correctly record and column ids, an overlap of 3 over 5 words in a cell value is a strong signal that is naturally captured by the walks over the graph.

Inspired from the reviewer's comment and from the new datasets with larger and noisier texts, we explored the trade-off between these two extremes and found an effective heuristic to get the best of both worlds.
Consider the ER process with two datasets. In our updated graph generation procedure, when a cell value is overlapping (or mergeable) between two datasets, we consider it as a single token (``Saving\_Private\_Ryan''). But, if the cell value is not overlapping between the two, we tokenize it into multiple words. The crucial point is that these multiple nodes in the graph are connected to the \textit{same row id} and to the \textit{same column id}. This preserves the inter-tuple and inter-attribute connections very naturally with no changes to any of the downstream algorithms in our solution.
We conducted new experiments to investigate this problem. 
The results from Table~4 shows that our proposed heuristic -- \textit{overlap} -- provides good results. 

%As an optimization, we keep modeling overlapping tokens between the two datasets ``as-is'' in the graph (e.g., ``Saving Private Ryan'' for a movie title) it is also increasing the quality of the integration over a solution where all words are modelled directly in the graph. 

\vspace{0.8ex}
\etitle{R5(D2).}
{\em Since one of the main problems addressed in this work is that of missing tokens in pre-trained vocabularies, Glove forms a weak baseline for this comparison. It would be much better to compare against approaches such as FastText which can generate embeddings for almost any token, even if it was never seen during training (this can be done using the fastText binary version, e.g.: https://dl.fbaipublicfiles.com/fasttext/vectors-crawl/cc.en.300.bin.gz).}

\stab
{\bf [A]}
%In Section~3, we identified a number of problems in pre-trained embeddings.
We agree with the reviewer that character based embeddings
could \emph{partially} alleviate the out-of-vocabulary issue. 
%\red{Paolo: clarify if the new pretrained results are from glove or fasttext!}
A local embedding trained on the actual data (enterprise or otherwise)
would necessarily have better embedding quality
than the approximation obtained by fastText through the embeddings of constituent n-grams.
Moreover, fastText will not be able to address the other issues such as
learning relationships inherent in the structured data that is needed for data integration tasks.
Prior work such as DeepER~\cite{deeper} (see Table~6)
found that varying the pre-trained embeddings (such as word2vec, GloVe, fastText)
had only a minor impact on the entity matching task.
We now report our experiments with fastText pretrained embeddings and show in Tables~3 and 4 that they do not outperform EDI.
%These experime can be found in Table~XYZ.
%\red{Paolo: we report only FT, glove was similar, we changed it to make this reviewer happy}


\vspace{5ex}
\noindent {\large\em Yours sincerely,}

\vspace{1.8ex}
{\large\em The authors}

\balance
\clearpage

